A light- and heat-seeking vine-inspired robot with material-level responsiveness

The fields of soft and bio-inspired robotics promise to imbue synthetic systems with capabilities found in the natural world. However, many of these biological capabilities are yet to be realized. For example, vines in nature direct growth via localized responses embedded in the cells of vine body, allowing an organism without a central brain to successfully search for resources (e.g., light). Yet to date, vine-inspired robots have yet to show such localized embedded responsiveness. Here we present a vine-inspired robotic device with material-level responses embedded in its skin and capable of growing and steering toward either a light or heat stimulus. We present basic modeling of the concept, design details, and experimental results showing its behavior in response to infrared (IR) and visible light. Our simple design concept advances the capabilities of bio-inspired robots and lays the foundation for future growing robots that are capable of seeking light or heat, yet are extremely simple and low-cost. Potential applications include solar tracking, and in the future, firefighting smoldering fires. We envision using similar robots to find hot spots in hard-to-access environments, allowing us to put out potentially long-burning fires faster.

==> modelingOG.tex <==
\section{Modeling og}
\label{sec:model}
To predict the pose of the robot in a given light or heat field requires the coupling of four models: a heat transfer model, a temperature-pressure model, a pressure-force-contraction ratio model, and a statics pose model. The heat transfer model allows us to find the temperature for each of the PPSAs distributed along the robot, given a light or heat flux. The temperature-pressure model enables us to relate the temperature of a given PPSA to its internal pressure. The pressure-force-contraction ratio model allows us to predict the force-contraction ratio relation for a single PPSA given a pressure. Finally, the statics pose model allows us to determine the shape of the robot based on the contraction ratios and forces produced by all of the PPSA pouches along the robot body (Figure \ref{fig:flow chart}). Additionally, the pose model could feed back into the heat transfer model, because the the pose of the robot might alter the heat transfer. For example, figure \ref{fig:first_fig}C shows how the robot alters the beam pattern of the light source. After presenting this four-part model, we describe how we implement it.
%Figure \ref{fig:flow chart} shows the modeling flow.


%Instead, we do a semi-empirical. 

\subsection{Four Components of the Model}
In this section, we describe the four components of the model: (i) flux-temperature model, which relates light flux to an individual PPSA temperature; (ii) temperature-pressure model, which relates the temperature of a PPSA to its internal pressure; (iii) the pressure-force-contraction ratio, which relates PPSA pressure to its force-contraction ratio curve; and (iv) the static pose model, which takes in the force-contraction ratio relationship of all of the PPSAs on the vine robot and outputs its pose.

\subsubsection{Flux-Temperature Model}

The development of an analytical model for the relationship between flux and PPSA temperature is not straightforward, due to the multi-material construction and complex geometries. These factors make it difficult to derive a closed-form solution for the heat transfer. Therefore, after introducing the relevant equations, we describe an empirical method for deriving this relationship, which we use in our model.
%in addition to presenting our three-part modeling, we also present a semi-empirical approach, in which we use experimental data to bypass the heat transfer model and directly relate light flux to the force-contraction ratio curve of a single PPSA, which can then be fed into the statics model to predict robot pose.

At equilibrium, a simple energy balance for the $i^{th}$ PPSA is  

\begin{equation}
    \sum_{j=1}^{N} h_{ij }(T_i-T_j)=\sum_{j=1}^{N} A_i F_{ij}(J_j-J_i) 
\end{equation}

$T_i$ is the effective temperature, $h_{ij}$ represents the combined conductive and convective heat transfer coefficient from PPSA $i$ to PPSA $j$, $A_i$ is the effective area of the PPSA, $F_{ij}$ is the effective view factor from PPSA $i$ to PPSA $j$, and $J$ is radiosity. 

A major challenge of this model is computing the view factors. The complex geometries and multi-material constructions make it hard to construct analytical and numerical solutions for all the reflections, refractions, re-radiation, etc.

Accordingly, we instead build an empirical relationship between flux and the effective temperature of a PPSA. We use a series of measurements to characterize how different flux magnitudes create different responses in PPSAs, and then interpolate between data points to form the relationship used in the model. Details of this process are described in Section \ref{sec:implementation}.

\subsubsection{Temperature-Pressure Model}
\label{sec:TP Model}
In this section, we use a model that describes the gauge pressure, $P_g$, inside a flexible pouch to model the gauge pressure inside the PPSA \cite{sanchez2020smart}
\begin{equation}
    P_g=
    \begin{cases} P_{PC}(T)+\frac{n_{air}RT}{V}-P_{atm}, & P_{PC}(T)+\frac{n_{air}RT}{V}>P_{atm}
    \\0, & P_{PC}(T)+\frac{n_{air}RT}{V} \leq P_{atm}
    \end{cases}
\end{equation}
$P_{PC}$, $T$, $n_{air}$, $R$, $V$, $P_{atm}$ are the Novec 7000 vapor pressure, absolute temperature, moles of residual air, ideal gas constant, actuator volume, and atmospheric pressure, respectively. The pressure terms on the right hand side are absolute pressures. If we assume that the residual air is negligible and that there is sufficient fluid, then the pressure inside the actuator depends only on temperature at equilibrium. We use the REFPROP database for our fluid model \cite{LEMMON-RP10}. 

\subsubsection{Pressure-Force-Contraction Ratio Model}
\label{sec:p-f-s Model}
The force exerted by a PPSA depends on the pressure and contraction ratio. Understanding how the force changes with pressure allows us to couple the temperature-pressure model (above) with the statics pose model (below).

An individual PPSA pouch acts as a pleated pneumatic artificial muscle (PPAM) \cite{daerden1999conception,daerden2001concept} or a single unit of a series pneumatic artificial muscle (sPAM) \cite{greer2017series}. While the model that describes the PPAM and sPAM is qualitatively useful, it does not adequately describe the friction effects observed in Fig. \ref{fig:ForceStrain}. The multi-layer Mylar film we use is noticeably less supple than than the polyethylene of \cite{greer2017series}, due to the requirement for it to be gas impermeable over long times scales (days). Therefore, we created an empirical model, measuring the force-compression curve at various pressures for sPAMs made of Mylar.

% \subsubsection{Temperature-force-contraction Ratio Model}
% \label{sec:t-f-s Model}
% The force exerted by a PPSA depends on the contraction ratio and temperature. Understanding how the force changes with temperature allows us to couple the heat transfer model (above) with the statics pose model (below). At a high level, we find that as temperature increases, the PPSA force at a given contraction ratio increases. We determine the details of this relationship from the model in this section, which is built upon the force-contraction ratio model for pleated pneumatic actuators (PPAMs) \cite{greer2017series,daerden1999conception,daerden2001concept} and a temperature-pressure model for phase-change textile actuators \cite{sanchez2020smart}.

% First, we can relate the internal pressure of the PPSA to its force-contraction ratio behavior. To do so, we first note that the individual units of the PPSAs behave similarly to pleated pneumatic artificial muscles \cite{daerden2001concept}, and can thus leverage models created for these pleated muscles. For a given contraction ratio of the active region, $\gamma$, the force, $F_{\gamma}$, produced is
%  \begin{equation}
% F_{\gamma}=\pi P_g r^2 \frac{1-2 m}{2 m \cos^2(\phi_r)}, \quad \frac{2r}{\cos(\phi_r)}<\frac{2w}{\pi}
% \label{eq:force}
%  \end{equation}

% $P_g$ is the gauge pressure inside the actuator, $r$ is the radius of the constriction, $w$ is the flat tubing width used for the actuator, $m$ and $\phi_r$ are parameters determined from the below system of equations. 
 
%  \begin{equation}
%  \begin{cases}\frac{F(\phi_r |m)}{\sqrt{m}\cos(\phi_r)}=\frac{l}{r}  \\ \frac{E(\phi_r |m)}{\sqrt{m}\cos(\phi_r)}=\frac{l}{r}(1-\frac{\gamma}{2})
%  \end{cases}
%  \end{equation}
 
% $F$ and $E$ are the first and second incomplete elliptic integrals, respectively.
% The condition on the right hand side of Equation \ref{eq:force} is the zero parallel force condition \cite{greer2017series,daerden2001concept}.
% For further discussion and derivation of the force-contraction pleated actuator model, see \cite{greer2017series}, \cite{daerden2001concept}, and \cite{daerden1999conception}.

% The second model that we leverage describes the gauge pressure inside a flexible pouch made from an inextensible material \cite{sanchez2020smart}. 
% \begin{equation}
%     P_g=
%     \begin{cases} P_{PC}(T)+\frac{n_{air}RT}{V}-P_{atm}, & P_{PC}(T)+\frac{n_{air}RT}{V}>P_{atm}
%     \\0, & P_{PC}(T)+\frac{n_{air}RT}{V} \leq P_{atm}
%     \end{cases}
% \end{equation}
% $P_{PC}(T)$, $T$, $n_{air}$, $R$, $V$, $P_{atm}$ are the Novec 7000 vapor pressure, absolute temperature, moles of residual air, ideal gas constant, actuator volume, and atmospheric pressure, respectively. The pressure terms on the right hand side are absolute pressures. Ideally, there is no residual air inside the actuator. 

% Combining these two models, we are able to predict the relationship among temperature, force, and contraction ratio for our PPSA. \ref{fig:ForceStrain} plots the model and experimental data. We expect that increasing temperature shifts the force-contraction ratio curve upward, increasing the force produced at a given contraction ratio. We also expect an inverse relationship between force and contraction ratio, and a pressure independent zero force contraction ratio (i.e., regardless of internal pressure, there is a contraction ratio for which no force is produced).



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/ModelingFlow2.png
    %ModelingFlow.png
    %ModelingFlow.png
    }
    \caption{Overview of the modeling framework. The black arrows are relationships directly modeled or measured and the grey arrows are the non-modeled relations}
    \label{fig:flow chart}
\end{figure}




\subsubsection{Static Pose Model}
In this section, we present a model that predicts the static pose of the robot given the force-contraction ratio of each of the PPSAs along the robot body. The contraction-ratio of each PPSA might vary due to possible temperature variations. The model shows that even though the contraction ratio and temperature of each PPSA may be different, the force exerted by each PPSA will be the same. This is because the tension in the PPSAs at a given cross section will be equal and opposite the axial expansion pressure inside the pneumatic backbone. 

For example, if the backbone is exerting an expansion force of 10N, each of the two PPSAs on either side will be applying 5N; however, the one that is closer to the light source and hotter will have a greater contraction ratio (see dotted line on Fig. \ref{fig:ForceStrain}).
%are pose-independent and that the shape is determined by the contraction ratio of PPSAs and the pressure inside the pneumatic backbone. 


%If it can be determined the relationship between light flux and PPSA temperature as well as between PPSA temperature and force-contraction ratio, the final step of the modeling is the statics model that predicts the pose of the robot given the force-contraction ratio curve of the PPSAs. Below, we provide the details of this model, which shows that the force in PPSAs on either side of the vine robot will be equal and determined by the pressure inside the main body of the robot, while the contraction ratio of these opposing PPSAs will be determined by their two different temperatures (and same force).


To form this statics pose model, we first discretize the vine robot body into a series of $N$ trapezoidal sections, each consisting of three springs (Figure \ref{fig:kinematicModel}).
The center spring represents the pneumatic axial expansion force, and the two outer springs represent the PPSAs. We assume there are no forces between the trapezoidal sections, because we assume the robot is free from external contacts (i.e., on a frictionless surface). We assume the torsion forces at the interfaces are minimal since the robot is locally buckled (cite). 

\begin{figure}[H]
    \centering
    \includegraphics[width=1\columnwidth]{Figures/SketchOfModel2.png}
    \caption{Detail of the static pose model. The outline of the robot is shown in light gray, the trapezoidal geometry and dimensions are shown in a darker gray, and the fores are shown in black}
    \label{fig:kinematicModel}
\end{figure}

The force and moment balances within the $i$-th section are respectively
\begin{equation}
    P_bA=f_{i,1}(\gamma_{i,1})+f_{i,2}(\gamma_{i,2})
\end{equation}
\begin{equation}
    f_{i,1}(\gamma_{i,1})=f_{i,2}(\gamma_{i,2})
\end{equation}
$P_b$ is the gauge pressure of the pneumatic backbone, $A$ is the cross-sectional area of the backbone, $f$ is the force exerted by the PPSA, and $\gamma$ is contraction ratio of the PPSA.
For static balance to occur $f_{i,1}(\gamma_{i,1})=f_{i,2}(\gamma_{i,2})=P_bA/2$.  The $i$-th angle can be determined from the relation
\begin{equation}
    l_0(1-\gamma_{i,2})+\frac{d}{\tan(\theta_{i-1})}+\frac{d}{\tan(\theta_i)}= l_0(1-\gamma_{i,1})
\end{equation}

 $d$ represents the width spacing between the two PPSAs. For simplicity, we assume this value is constant. To initialize the problem, we assume $\theta_0=\pi/2$. 
The coordinates of the points on the $1$ side (e.g., the side facing the light) of the robot are:
\begin{equation}
y_{i,1}=\sum_{j=1}^{i} \Big(l_{1,i} \cos\big(\sum_{k=0}^{i-1} (\pi-2\theta_k)\big)\Big)
\end{equation}

\begin{equation}
x_{i,1}=\sum_{j=1}^{i} \Big(l_{1,i} \sin\big(\sum_{k=0}^{i-1} (\pi-2\theta_k)\big)\Big)
\end{equation}
A similar expression can be derived for the $2$ side of the robot.

This model tells us that at equilibrium, the force exerted by each PPSA depends solely on the pressure of the pneumatic backbone and is independent of temperature. However,  the exact strain state (i.e., $\gamma$) of a certain PPSA depends on the pneumatic backbone pressure and the temperature of the PPSA. 
%requires additional information. It can be modeled or empirically determined.

% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{Figures/model_flowchart1.png}
%     \caption{Steps taken to achieve model in Figure \ref{fig:ModelVerificaiton}.}
%     \label{flow chart}
% \end{figure*}






  
\subsection{Implementation}
\label{sec:implementation}
To implement the presented model, we require data to build the empirical models that relate light flux to PPSA temperature (Model Part 1) and that relate pressure to a force-contraction ratio curve (Model Part 3). Model Part 2 (Temperature-pressure) is based on the literature and Model Part 4 (Static Pose) is analytical, so these do not require data gathering for implementation. Below we describe the series of measurements and calculations, performed for Model Part 1 and 3.
%As long as a relationship between a quantity and distance or strain exists, then other relations such as flux vs. strain can be derived. 


For Model Part 1, we first measured the relationship between distance to the light source and flux. Next, we measured the relationship between distance from the light source and PPSA contraction ratio at an arbitrary force level (we chose 5 N). Finally, we used Model Part 2 (temperature-pressure) and Model Part 3 (pressure-force-contraction ratio, see below)to determine an effective temperature for each measured force-contraction ratio data point. With this set of measurements and calculations, we were able to relate the light flux to effective temperature in the PPSA, the goal of the first step of the model.  Although this model works for simple cases, its efficacy is limited in more complex scenarios (e.g., scenes with shading), because the boundary conditions for each of the PPSAs will differ from the ones used to determine the empirical relations.
In these cases, a fully analytical or computational heat transfer model would be beneficial.
%The first step of the implementation uses an experimentally determined relationship between distance and the strain state of the PPSAs. 
%From the static pose model, we know that at equilibrium, the force exerted by the PPSAs is pose-independent.
%To acquire this data we measured the strain required to exert \SI{5}{\newton} (arbitrarily chosen) as a function of distance.
We present the data and details from the above experiments in Section \ref{sec:Contraction Ratio vs. Flux}.

However, for simple cases without self-shadowing, we can use this relationship to now take an arbitrary flux field and predict the effective temperature of each pouch. From there, using Model Part 2, we can predict the pressure, and then with Model Part 3, the force-contraction ratio relationship for each pouch. Then, using Model Part 4 and a given backbone pressure, we can predict the force and contraction ratio of each PPSA pouch and thus the pose of the entire robot. 
We show the results of our predictions compared to actual experimental poses in Section \ref{sec:verification}.

% \begin{figure}
%     \centering
%     \includegraphics[width=.8\columnwidth]{Figures/FD_PPSA.pdf}
%     \caption{The vine robot body requires a roughly constant 5 N of force applied by a PPSA to bend it through the range of angles expected during use. Therefore, in our model, we assume a fixed force on each active PPSA, and thus can relate light flux to strain state for this force level using our gathered data.}
%     \label{fig:FD_PPSA}
% \end{figure}

==> resultsOG.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Results}
In this section, we first describe the experiments used to determine the empirical relationship for the first component of the model (flux to PPSA temperature). Next, we present experimental validation of the second component of the model, the temperature-force-contraction ratio model. Then, we validate the full 3-part model, predicting three different poses in three different light flux fields. Finally, we show demonstrations of the phototropic vine robots seeking light sources. 
%Heat transfer in radiative systems is often environmentally and configurationally dependent. To characterize the performance of our actuators, we varied the strain on the actuator and measured the corresponding force under different environmental conditions.  
%We first tested them in a constant-temperature environment (Figure \ref{fig:inbox_schematic}) before testing them in a relatively uncontrolled environment (lab space) under different illumination conditions (Figures \ref{fig:outbox_schematic},\ref{fig:Simple Environment}). 
For each actuation test, we used PPSAs comprised of five pouches to minimize the effects of any potential manufacturing variations in a single pouch. 

\subsection{Determination of Model Part 1: Empirical Relationship between Flux and Temperature}
To determine the first component of the 3-part model, we conducted a series of measurements, described below.

\subsubsection{Flux versus Distance from Light}
We first estimated the relationship between flux and distance from the light source. This allowed us in the following experiment to estimate how much flux each PPSA was experiencing as we varied the distance to the light. We determined this relationship by measuring the equilibrium temperature, $T_{plate}$, of a black-painted aluminum plate ($\sim$\SI{1.6}{\centi\meter} $\times$ \SI{1.6}{\centi\meter}) as we varied its distance from the light. The center of plate was placed ~\SI{2}{\centi\meter} above the polystyrene floor, which is approximately level with sPAMs on the robot. For simplicity, we assume the plate is a blackbody and use a vertical flat plate convection model \cite{bergman2011fundamentals} to estimate the flux as:
$Q_{light}=\sigma T_{plate}^4-h(T_{plate}-T_{amb})$. As expected, the flux roughly obeys the inverse square law. Using IR imaging (FLIR E60) we determined spatial distribution of heat around the lamp and found good agreement with the model (Figure \ref{fig:Simple Environment}).  





\begin{figure}[tb]
    \centering
    
    \includegraphics[width=1.0\columnwidth]{Figures/HeatFluxMeasure.png}
    \caption{\textbf{A:} Flux as a function of distance. The circles are the experimentally measured points and the solid line is an exponential fit to the data. \textbf{B:} IR image of the temperature produced by lamp on a polystyrene foam floor. The contours represent isotherms, which we interpret as isoflux lines.}
    \label{fig:Simple Environment}
\end{figure}



 
  \begin{figure}
  \begin{center}
  \includegraphics[width=.9\columnwidth]{Figures/fluxSensing.png}
  \caption{Image of flux testing setup. 
  }
  \label{fig:outbox_schematic}
  \end{center}
  \vspace{-5mm}
\end{figure}




\subsubsection{Contraction Ratio versus Distance from Light}
\label{sec:Contraction Ratio vs. Flux}
Next, we measured the contraction ratio at different distances from the light at predetermined force level. 
A 5-pouch PPSA was suspended by two pieces of Spectra fiber (\textit{Power Pro} 80 lb test). One end of the fiber was pinned and the other was
attached to a force gauge (Mark-10 M3-5) on a translating stage. We use a quartz lamp (Infratech W-7512 SS) with an approximate emission wavelength peak of \SI{3.2}{\micro\meter}.(Figure \ref{fig:outbox_schematic}).
%To measure the force-strain relationship, we build a simple tensile test setup made up of styrofoam placed upon an acrylic board of dimensions (X by Y cm) (Fig. \ref{fig:outbox_schematic}). Two pieces of Spectra fiber (\textit{Power Pro} 80 lb test) are used to suspend an actuator above the styrofoam, of which one of the strings is attached to a force gauge (Mark XX) (500 N) and the other is tied to a screw. The top nut on the screw is used to position the string such that when the actuator just becomes taut, it is parallel to the ground. Before starting the experiment, the bottom nut (refer to figure) is loosened to adjust the screw across a slot rail on the acrylic board. Once the length of the set of pouches is measured to be that at manufacture, the nut is tightened. 
The PPSA was backed with a \SI{5}{\centi\meter} diameter LDPE tubing to simulate the heat transfer effects of the central spine.
%Styrofoam spacers of width 5 and 10 cm are used to arrange the actuator at various distances from the front face of the heater. 
In each test, the system was equilibrated for 12 minutes to reach steady state and the screw displacement required to produce  \SI{5}{\newton} of force was measured. This allowed the contraction ratios to be measured as a function of distance (Figure \ref{fig:StrainTo5N}).


%mention that as the pouches contracted, the setup is shifted so that the center pouch of the set of 5 was aligned with the midpoint of the heater to ensure more or less constant flux. The strain is calculated as the ratio of the displacement of the screw, to the free length of the actuator. 

%According to the kinematic model, at equilibrium, the force exerted by the sPAMs on each side of the robot are equal and proportional to the pressure inside the body. 

%For our tests, we arbitrarily chose \SI{5}{\newton} as the required deformation force. the heater and the sPAMs, we use a series of styrofoam spacers. 

\subsubsection{Assembling Components to Relate Flux to Temperature}
Toward the goal of relating flux to temperature, we first combine the above sets of data to relate contraction ratio to flux (flux versus distance shown in Fig. \ref{fig:Simple Environment}A and contraction ratio versus distance shown in Fig. \ref{fig:StrainTo5N}). We can then create an empirical model of contraction ratio versus flux, shown in Fig. \ref{fig:StrainTo5N}B.
At low flux values, the required contraction ratio varies nearly linearly with flux, then saturates at higher flux values to an upper limit that is determined by the pressure-independent zero force contraction ratio. Thus higher fluxes, which result in higher equilibrium temperatures and pressures, cannot increase contraction ratios indefinitely.

Finally, we use the temperature-force-contraction ratio model to determine the effective temperature for any given pair of force and contraction ratios. This allows us to plot the desired relationship of effective temperature versus flux (Fig. XX). 


\begin{figure}[H]
    \centering
    \includegraphics[width=1\columnwidth]{Figures/strainTo5N2_2.png}
    \caption{Contraction ratios required to achieve \SI{5}{\newton} of force as a function of (A) distance and (B) flux.}
    \label{fig:StrainTo5N}
\end{figure}

%[some figure] shows the strain interpolated from the measurements as a function of distance from the heater. 






%\subsection{Verification of Model Part 2: Temperature-Force-Contraction Ratio Model}

 %\begin{figure}
  %\begin{center}
  %\includegraphics[width=.7\columnwidth]%{Figures/InBoxNoSchematicMoreCompressed.png}
  %\caption{Schematic showing an image the temperature-controlled experimental setup, with PPSA position indicated by red dotted lines.
  %}
  %\label{fig:inbox_schematic}
  %\end{center}
  %\vspace{-7mm}
%\end{figure}

%To verify the second part of the model, we measured the force versus contraction ratio relationship as temperature was varied. We placed a 5-pouch PPSA in a temperature controlled box, suspended by two pieces of Spectra fiber. As in the previous experiment, one end of the fiber was pinned and the other was attached to a force gauge on a translating stage (Figure \ref{fig:inbox_schematic}). To find the free length of the actuator, we translated the linear stage at room temperature ($\sim$\SI{20}{\celsius}) until the PPAM transitioned from slack (\SI{0}{\newton}) to slightly tensioned (\SI{2.8}{\newton}). The contraction ratio was varied by translating the linear stage to differing positions. Figure \ref{fig:ForceStrain} shows the force-contraction ratio relations produced by the PPSA at two different temperatures, along with the model from Section \ref{sec:t-f-s Model}. As predicted, force increases with temperature and varies inversely with contraction ratio, and the zero force contraction ratios are nearly the same. 



\subsection{Pressure-Force-Compression Relations}
\begin{figure}[tb]
    \centering
    \includegraphics[width=1\columnwidth]{Figures/Mylar_sPAM.png}
    \caption{Force vs. contraction ratios for different pressures.}
    \label{fig:ForceStrain}
\end{figure}

To obtain the relations, we measured the force versus contraction ratio relationship for an sPAM made of Mylar under varying pressures.  

We mounted the sPAM onto a linear stage and varied the contraction ratio by  translating the stage (Figure \ref{fig:inbox_schematic}). A force transducer recorded the forces. We measured both the extension and contraction of the sPAM. To find the free length of the actuator, we translated the linear stage ($\sim$\SI{20}{\celsius}) until the sPAM transitioned from slack (\SI{0}{\newton}) to slightly tensioned (\SI{2.8}{\newton}). 

Fig. \ref{fig:ForceStrain} shows the force-contraction ratio relations produced by the Mylar sPAM at different pressures. 

Qualitatively, the shape of the curves matches that of the PPAM and sPAM. However, the model in \cite{daerden1999conception,daerden2001concept,greer2017series} over-predicts the forces. Notab

\subsection{Verification of Full 3-part Model}
\label{sec:verification}
We next tested the full 3-part model by comparing the predicted deformation of a short section of a phototropic vine robot to experimental values (Figure \ref{fig:ModelVerificaiton}). With respect to the center of the PPSA on the heater side, the robot was placed \SI{55}{\centi\meter} away from the heater. The center body was inflated to about \SI{12}{\kilo\pascal}, so that the required deformation force is \SI{5}{\newton}. To estimate the contraction ratio at this distance, we interpolated the data presented in Figure \ref{fig:StrainTo5N}A to find $\gamma=0.163$. Setting $l_0=$ \SI{4.1}{\centi\meter}, $d=$ \SI{5.0}{\centi\meter}, and $\theta_0=\pi/2$, we computed the expected PPSA shape. When the computed shape is overlaid on the experimental image, there is good agreement, validating the utility of the model. In this approach, the PPSA positioned away from the heater is assumed to be sufficiently insulated that $\gamma=0$, while the PPSA on the heater side is uniformly illuminated, which is consistent with infrared imaging results of a similar test (inset). We attribute the small discrepancies to unmodeled dimensional variations in the constructed PPSAs and heat transfer to the antagonistic side. It is possible that the changes in view factors and flux as the robot deforms, which are assumed to be small, also contribute to some extent. 
  

%We tested the model under simple illumination conditions because of the uncertainty in how robot pose affects illumination on the sPAMs.


%\section{Results}
% Our experiments are divided into light free and light-based tests. 

% For our light-based tests, our setup is as following

% sPAM characterization. Mention how we test multiple units at once to average out manufacturing effects

% \label{sec:Results}






%\subsection{Kinematic Model Verification}
%Figure \ref{fig:ModelVerificaiton} compares our kinematic model predictions to the experiment. Overall, there is good agreement. Most of the discrepancies can be explained by the unmodeled dimensional variations in the constructed sPAMS.




\begin{figure}[tb]
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/ModelVerificationWithCorrected.png}
    \caption{Model verification on a section of robot. The predicted shape is drawn in orange. Inset shows the infrared image of a similar test setup.}
    \label{fig:ModelVerificaiton}
    \vspace{-5mm}
\end{figure}


\subsection{Demonstration}
We demonstrate the robot growing via internal pressure and steering with the PPSAs toward the light source in three different scenarios. The light is relatively low power, with the flux that reaches the robot ranging from approximately 0.1-0.5 that of the sun. Figure \ref{fig:demo}C shows that the robot can find the light source even if it is initially growing away from it. Figure \ref{fig:demo}B and C shows the robot navigating around simple obstacles. It is possible to increase the steering speed by placing the robot closer to the light source ($\sim$\SI{35}{\centi\meter}), as shown in  Figure \ref{fig:speedTest} where $\sim$\SI{90}{\second} reorientation times are achieved. Notably, in this case, we demonstrate the turning process without eversion. Since the robot is significantly stiffer when there are PPSAs inside the spine, a higher actuation force is required, which takes longer to achieve.


% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.3\textwidth]{Figures/stress-strain.png}
%     \caption{will be a surface (3D)}
%     \label{fig:stress-strain}
% \end{figure}

% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=1.0\columnwidth]{Figures/draftFig3.png}
%     \caption{A: Force strain graph at various temperatures. B: Force strain measurement setup. C: Effective temperature plot D. Effective temperature vs angle plot}
% \end{figure}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{Figures/video_demos_betterres.png}
\vspace{-3mm}
\caption{Demonstrations of thermotropic eversion toward the indicated heat source in unknown environments. The PPSAs actuate asymmetrically under thermal activation, enabling the robot to bend and grow in a path defined by the styrofoam barriers. \textbf{A:} Eversion of one vine robot towards a heater on the right. \textbf{B:} Eversion of two vine robots towards the same heater. \textbf{C:} Eversion of two vine robots towards two heaters on the left and right. }
\label{fig:demo}
\vspace{-2mm}
\end{figure*}


\begin{figure}[tb]
\centering
\includegraphics[width=1.0\columnwidth]{Figures/speedTest2_2.png}
\vspace{-5mm}
\caption{The robot can steer towards the heat source within \SI{90}{\second}}
\label{fig:speedTest}
\vspace{-5mm}
\end{figure}

